Communication-Efficient Topologies for Decentralized Learning with $O(1)$ Consensus Rate

Decentralized optimization is an emerging paradigm in distributed learning in which agents achieve network-wide solutions by peer-to-peer communication without the central server. Since communication tends to be slower than computation, when each agent communicates with only a few neighboring agents per iteration, they can complete iterations faster than with more agents or a central server. However, the total number of iterations to reach a network-wide solution is affected by the speed at which the agents' information is ``mixed'' by communication. We found that popular communication topologies either have large maximum degrees (such as stars and complete graphs) or are ineffective at mixing information (such as rings and grids). To address this problem, we propose a new family of topologies, EquiTopo, which has an (almost) constant degree and a network-size-independent consensus rate that is used to measure the mixing efficiency. In the proposed family, EquiStatic has a degree of $\Theta(\ln(n))$, where $n$ is the network size, and a series of time-dependent one-peer topologies, EquiDyn, has a constant degree of 1. We generate EquiDyn through a certain random sampling procedure. Both of them achieve an $n$-independent consensus rate. We apply them to decentralized SGD and decentralized gradient tracking and obtain faster communication and better convergence, theoretically and empirically. Our code is implemented through BlueFog and available at \url{https://github.com/kexinjinnn/EquiTopo}

==> dsgd.tex <==
Here the convergence properties of the decentralized stochastic gradient descent algorithm are analyzed.

For simplification, we introduced some notations as follows.

\begin{itemize}[leftmargin = 1.5em]
\item $\X^{(t)} = [(\x_1^{(t)})^T; (\x_2^{(t)})^T; \cdots; (\x_n^{(t)})^T] \in \R^{n \times d}$;
\item $\bX^{(t)} = \big[(\bar{\x}^{(t)})^T; (\bar{\x}^{(t)})^T; \cdots; (\bar{\x}^{(t)})^T \big]\in \R^{n \times d}$;
\item $\g^{(t)}=  \big[\nabla F_1(\x_1^{(t)}; \xi_1^{(t)})^T; \nabla F_2(\x_2^{(t)}; \xi_2^{(t)})^T \cdots; 
\nabla F_n(\x_n^{(t)}; \xi_n^{(t)})^T \big] \in \R^{n \times d}$;
\item $\tf^{(t)}= \big[\nabla f_1(\x_1^{(t)})^T; \nabla f_2(\x_2^{(t)})^T \cdots; 
\nabla f_n(\x_n^{(t)})^T \big] \in \R^{n \times d}$;
\end{itemize}

Clearly, Algorithm \ref{dsgd} can be simplified as 
\begin{equation}
\label{alg_sim}
\X^{(t+1)} = \W^{(t)} \big(\X^{(t)} - \gamma \g^{(t)} \big), ~~ \X^{(0)} = \bX^{(0)}.
\end{equation}	

Referring to Lemma 6 of \cite{chen2021accelerating}, we have the following descent lemma for \ref{alg_sim}.

\begin{lemma}
\label{lem:descent}
(DESCENT LEMMA)
Let Assumptions A.1-A.3 hold.
Suppose that $\W^{(t)}$ is doubly stochastic for any $t$.
If $\gamma < 1/(4L)$, then
$$
\E \big[ f(\bar \x^{(t+1)}) \big] \le \E  \big[f(\bar \x^{(t)})\big] - \frac \gamma 4 \E \Big [\norm{\nabla f(\bar \x^{(t)})}^2  \Big]
+ \frac{3\gamma L^2}{4n} \E \Big[  \norm{\X^{(t)} - \bar \X^{(t)}}_F^2 \Big] + \frac {\gamma^2 \sigma^2 L}{2n}
$$
where $\norm{\cdot}_F$ means Frobenius norm.
\end{lemma}	

Moreover, we have the following running consensus lemma for (\ref{alg_sim}).
\begin{lemma}
\label{runningnonconv}	
(RUNNING CONSENSUS LEMMA)
Let Assumptions A.1- A.3 holds.	Suppose that $\W^{(t)}$ is doubly stochastic for any $t$, and moreover,
$\E[\norm{\Pin \W^{(t)} \y}] \le \beta \norm{\Pin \y}$ for all $\y\in \R^n$.
If $\gamma< $, then
\begin{equation*}
\begin{aligned}
\frac {1}{T+1} \sum_{t=0}^T \E \Big[\norm{ \X^{(t)} - \bX^{(t)}}_F^2 \Big] \le  
\frac {6 n\gamma^2 \beta^2}{(1-\beta)^2 (T+1)}\sum_{t=0}^T \E\Big[\norm{\nabla f(\bar \x^{(t)})}^2 \Big]
+\frac{2 n \gamma^2 \beta^2}{1-\beta} \Big(\sigma^2 + \frac {3 b^2}{1-\beta} \Big).
\end{aligned}		
\end{equation*}	
\end{lemma}	

\emph{Proof.}
We first prove a bounds for $\E \big[ \norm{ \X^{(t+1)} - \bX^{(t+1)}}_F^2\big]$.

It follows from (\ref{alg_sim}) that
$$
\E \Big[ \norm{ \X^{(t+1)} - \bX^{(t+1)}}_F^2 | \mathcal F^{(t)}\Big] \\
=\E \Big[ \norm{(\W^{(t)}- \J)\big(\X^{(t)} - \bX^{(t)} - \gamma \g^{(t)}\big)}_F^2 | \mathcal F^{(t)} \Big].
$$
Due to Assumption A.2, 
\begin{equation*}
\begin{aligned}
\E &\Big[ \norm{ \X^{(t+1)} - \bX^{(t+1)}}_F^2 | \mathcal F^{(t)}\Big] \\
&=\norm{(\W^{(t)}- \J)\big(\X^{(t)} - \bX^{(t)} -\gamma  \tf^{(t)} \big)}^2
+\gamma^2 \E \Big[ \norm{(\W^{(t)}- \J)\big(\g^{(t)}- \tf^{(t)} \big)}_F^2  | \mathcal F^{(t)} \Big] \\
\end{aligned}		
\end{equation*}	

Notice that $\E[\norm{\Pin \W^{(t)} \y}] \le \beta \norm{\Pin \y}$ for all $\y\in \R^n$. 
Moreover, $\W^{(t)}$ is independent of $\X^{(t)}$.
By taking expectation over the filtration $\mathcal F^{(t)}$, we derive
\begin{equation*}
\begin{aligned}
\E \Big[ \norm{ \X^{(t+1)} - \bX^{(t+1)}}_F^2\Big] 
\le& \beta^2 \E \Big[\norm{(\big(\X^{(t)} - \bX^{(t)} -\gamma  \tf^{(t)} \big)}^2 \Big]
+\beta^2 \gamma^2 \E \Big[ \norm{\big(\g^{(t)}- \tf^{(t)} \big)}_F^2  \Big]\\
\le &\beta^2 \E \Big[\norm{(\big(\X^{(t)} - \bX^{(t)} -\gamma  \tf^{(t)} \big)}^2 \Big] + n\sigma^2 \beta^2 \gamma^2
\end{aligned}		
\end{equation*}	

Recalling Jensen inequality gives
\begin{equation*}
\begin{aligned}
\norm{\X^{(t)} - \bX^{(t)} -\gamma  \tf^{(t)}}^2
\le \frac {1}{t} \norm{\X^{(t)} - \bX^{(t)}}_F^2
+ \frac {\gamma^2}{1-t} \norm{\tf^{(t)}}_F^2.
\end{aligned}		
\end{equation*}	

Taking  $t=\beta$, and combining the above two inequalities, we derive
\begin{equation*}
\begin{aligned}
\E \Big[ \norm{ \X^{(t+1)} - \bX^{(t+1)}}_F^2\Big] \le
\beta \E \Big[ \norm{\X^{(t)} - \bX^{(t)}}_F^2 \Big] + \frac {\beta^2 \gamma^2}{1-\beta} \E\Big[ \norm{\tf^{(t)}}_F^2 \Big]
+ n\sigma^2 \beta^2 \gamma^2.
\end{aligned}		
\end{equation*}			

Furthermore, we have
\begin{equation*}
\begin{aligned}
\norm{\tf^{(t)}}_F^2 
&= \sum_{i=1}^n \norm{\nabla f_i(\x_i^{(t)})- \nabla f_i(\bar \x^{(t)}) + \nabla f_i(\bar \x^{(t)})
- \nabla f(\bar \x^{(t)})+  \nabla f(\bar \x^{(t)})}_F^2 \\
&\le 3L^2 \norm{\X^{(t)} - \bX^{(t)}}_F^2 + 3nb^2 +  3n\norm{\nabla f(\bar \x^{(t)})}^2.
\end{aligned}		
\end{equation*}			

Combining the above inequalities, we obtain
\begin{equation*}
\begin{aligned}
\E \Big[ \norm{ \X^{(t+1)} - \bX^{(t+1)}}_F^2\Big] \le&
\beta \E\Big[\norm{ \X^{(t)} - \bX^{(t)}}_F^2 \Big]
+ \frac {3\gamma^2  \beta^2 L^2}{1-\beta} \E\Big[\norm{ \X^{(t)} - \bX^{(t)}}_F^2 \Big] \\
&+\frac {3n\gamma^2 \beta^2}{1-\beta}  \E\Big[\norm{\nabla f(\bar \x^{(t)})}^2 \Big] 
+n \gamma^2 \beta^2 \Big(\sigma^2 + \frac {3 b^2}{1-\beta} \Big)
\end{aligned}		
\end{equation*}	

By setting $\X^{(0)} = \bX^{(0)}$, we derive
\begin{equation}
\begin{aligned}
\label{onestepdes:inenonconv}
\E \Big[ &\norm{ \X^{(t+1)} - \bX^{(t+1)}}_F^2 \Big]\\
\le& \frac {3\gamma^2 \beta^2 L^2}{1-\beta}\sum_{s=0}^t \beta^{t-s} \E \Big[\norm{\X^{(s)} - \bX^{(s)}}_F^2\Big] 
+\frac {3 n\gamma^2 \beta^2}{1-\beta}  \sum_{s=0}^t  \beta^{t-s} \E\Big[\norm{\nabla f(\bar \x^{(s)})}^2 \Big]\\
&+n \gamma^2 \beta^2 \Big(\sigma^2 + \frac {3 b^2}{1-\beta} \Big) \sum_{s=0}^t \beta^s
\end{aligned}		
\end{equation}	

In the following, we show the inequality in Lemma \ref{runningnonconv}.

For simplification, we define 
$$
D_1^{(t)}=\E \Big[\norm{ \X^{(t)} - \bX^{(t)}}_F^2 \Big],~~
D_2^{(t)}=\E\Big[\norm{\nabla f(\bar \x^{(t)})}^2 \Big],
$$
and moreover, 
$$
c_1=  \frac {3\gamma^2 \beta^2 L^2}{1-\beta},~~
c_2=\frac {3 n\gamma^2 \beta^2}{1-\beta},~~
c_3=\frac{2 n \gamma^2 \beta^2}{1-\beta} \Big(\sigma^2 + \frac {3 b^2}{1-\beta} \Big).
$$

Recalling (\ref{onestepdes:inenonconv}) gives
\begin{equation*}
\begin{aligned}
D_1^{(t)} &\le c_1 \sum_{s=0}^{t-1} \beta^{t-1-s} D_1^{(s)} +  c_2 \sum_{s=0}^t  \beta^{t-1-s} D_2^{(s)} +c_3.
\end{aligned}		
\end{equation*}	

Clearly,
\begin{equation*}
\begin{aligned}
\sum_{t=1}^T  D_1^{(t)} &\le c_1 \sum_{t=1}^T\sum_{s=0}^{t-1} \beta^{t-1-s} D_1^{(s)} +  c_2 \sum_{t=1}^T\sum_{s=0}^t  \beta^{t-1-s} D_2^{(s)} +c_3 T\\
&\le c_1 \sum_{s=0}^{T-1} D_1^{(s)}  \sum_{t=0}^{T-1-s}\beta^t
+  c_2 \sum_{s=0}^{T-1} D_2^{(s)}  \sum_{t=0}^{T-1-s}\beta^t +c_3 T \\
&\le \frac {c_1}{1-\beta} \sum_{s=0}^{T-1} D_1^{(s)}  
+ \frac {c_2}{1-\beta} \sum_{s=0}^{T-1} D_2^{(s)} +c_3 T
\end{aligned}		
\end{equation*}	

Note that $D_1^{(0)} = 0$. Therefore,
\begin{equation*}
\begin{aligned}
\sum_{t=0}^T D_1^{(t)} \le  \frac {c_1} {1-\beta} \sum_{t=0}^T D_1^{(t)} 
+  \frac {c_2} {1-\beta} \sum_{t=0}^{T}  D_2^{(t)} +c_3(T+1).
\end{aligned}		
\end{equation*}	

Take $\gamma = \frac {1-\beta}{3\beta L}$. Then $1-  \frac {c_1} {1-\beta} \ge \frac 12$, and as a result,
$$
\sum_{t=0}^T D_1^{(t)} \le  
\frac {2c_2} {1-\beta} \sum_{s=0}^t  D_2^{(s)} +2 c_3(T+1)
$$

Thus,
\begin{equation*}
\begin{aligned}
\frac {1}{T+1} \sum_{t=0}^T \E \Big[\norm{ \X^{(t)} - \bX^{(t)}}_F^2 \Big] \le  
\frac {6 n\gamma^2 \beta^2}{(1-\beta)^2 (T+1)}\sum_{t=0}^T \E\Big[\norm{\nabla f(\bar \x^{(t)})}^2 \Big]
+\frac{2 n \gamma^2 \beta^2}{1-\beta} \Big(\sigma^2 + \frac {3 b^2}{1-\beta} \Big).
\end{aligned}		
\end{equation*}	
The proof is completed.


~


\textbf{Proof of Theorem \ref{the:dsgd}}

Here the same notations as the proof of Lemma \ref{runningnonconv} are adopted.
It follows from Lemma \ref{lem:descent} that
$$
D_2^{(t)}\le \frac {4}{\gamma} \E  \big[f(\bar \x^{(t)})\big] - \frac {4}{\gamma}\E \big[ f(\bar \x^{(t+1)}) \big]
+ \frac{3 L^2}{n} D_1^{(t)} + \frac {2\gamma \sigma^2 L}{2n}.
$$


Taking running average over the above inequality, we obtain
\begin{equation*}
\begin{aligned}
\frac{1}{T+1}&\sum_{t=0}^T D_2^{(t)}
\le \frac {4}{(T+1)\gamma} \big[ f(\bar \x^{(0)}) - f(\x^*)\big]
+ \frac{3 L^2}{(T+1)n}\sum_{t=0}^T  D_2^{(t)} + \frac {2\gamma L\sigma^2}{n}.
\end{aligned}		
\end{equation*}	

Recalling Lemma \ref{runningnonconv} gives
\begin{equation*}
\begin{aligned}
\frac{1}{T+1}\sum_{t=0}^T D_2^{(t)}
\le  \frac {4}{(T+1)\gamma}   \big[ f(\bar \x^{(0)}) - f(\x^*)\big] 
+ \frac {6c_2 L^2} {n(1-\beta)(T+1)}\sum_{t=0}^T D_2^{(t)}
+\frac {6c_3 L^2} {n} + \frac {2\gamma L\sigma^2}{n}.
\end{aligned}		
\end{equation*}	
Take $\gamma \le \frac {(1-\beta)}{6\beta L}$. Then $ \frac {6c_2 L^2} {n(1-\beta)} \le \frac 12$, and as a result,
$$
\frac{1}{T+1}\sum_{t=0}^T \E\Big[\norm{\nabla f(\bar \x^{(t)})}^2 \Big] \le 
\frac {8}{(T+1)\gamma}   \big[ f(\bar \x^{(0)}) - f(\x^*)\big] 
+ \frac {4\gamma \sigma^2 L}{n} +\frac {12c_3 L^2} {n} .
$$

For simplification, we define
$$
r_0 = 8 \big[ f(\bar \x^{(0)}) - f(\x^*)\big],~~
r_1 = \frac {4 \sigma^2 L}{n}, ~~
r_2 =  \frac {12c_3 L^2} {n}.
$$

Then
$$
\frac{1}{T+1}\sum_{t=0}^T \E\Big[\norm{\nabla f(\bar \x^{(t)})}^2 \Big] \le \frac {r_0}{(T+1)\gamma} 
+r_1 \gamma +r_2 \gamma^2.
$$

Set $\gamma = \min \Big\{ \frac {1}{4L},  \frac {1-\beta}{3\beta L},  
\big (\frac {r_0}{r_2(T+1)} \big)^{\frac 13}, \big (\frac {r_0}{r_1(T+1)} \big)^{\frac 12} \Big\}$.
We discuss the convergence rate as follows.

\begin{itemize}
\item If $\big (\frac {r_0}{r_2(T+1)} \big)^{\frac 13} \le \big (\frac {r_0}{r_1(T+1)} \big)^{\frac 12}$,
we take $\gamma = \big (\frac {r_0}{r_2(T+1)} \big)^{\frac 13}$.
Then
$$
\frac{1}{T+1}\sum_{t=0}^T \E\Big[\norm{\nabla f(\bar \x^{(t)})}^2 \Big] \le  
2r_2^{\frac 13}\Big (\frac {r_0}{T+1} \Big)^{\frac 23} + \Big (\frac {r_0 r_1}{T+1} \Big)^{\frac 12}.
$$

\item If $\big (\frac {r_0}{r_1(T+1)} \big)^{\frac 12} \le \big (\frac {r_0}{r_2(T+1)} \big)^{\frac 13}$,
we take $\gamma=\big (\frac {r_0}{r_1(T+1)} \big)^{\frac 12}$. Then
$$
\frac{1}{T+1}\sum_{t=0}^T \E\Big[\norm{\nabla f(\bar \x^{(t)})}^2 \Big] \le  
2 \Big (\frac {r_0 r_1}{T+1} \Big)^{\frac 12} + r_2^{\frac 13} \Big (\frac {r_0}{T+1} \Big)^{\frac 23}.
$$

\item
If $\frac {1-\beta}{3\beta L} \le \big (\frac {r_0}{r_1(T+1)} \big)^{\frac 12}$, and moreover, 
$\frac {1-\beta}{3\beta L} \le \big (\frac {r_0}{r_2(T+1)} \big)^{\frac 13}$, we take 
$\gamma = \frac {1-\beta}{3\beta L}$. Then
$$
\frac{1}{T+1}\sum_{t=0}^T \E\Big[\norm{\nabla f(\bar \x^{(t)})}^2 \Big] \le  
\frac {3\beta L r_0}{(T+1)(1-\beta)} + \Big(\frac {r_0 r_1}{T+1} \Big)^{\frac 12}
+ r_2^{\frac 13} \Big (\frac {r_0}{T+1} \Big)^{\frac 23}.
$$

\item
If $\frac {1}{4L} \le \big (\frac {r_0}{r_1(T+1)} \big)^{\frac 12}$, and moreover, 
$\frac {1-\beta}{4L} \le \big (\frac {r_0}{r_2(T+1)} \big)^{\frac 13}$, we take 
$\gamma = \frac {1}{4L}$. Then
$$
\frac{1}{T+1}\sum_{t=0}^T \E\Big[\norm{\nabla f(\bar \x^{(t)})}^2 \Big] \le  
\frac {4 L r_0}{(T+1)} + \Big(\frac {r_0 r_1}{T+1} \Big)^{\frac 12}
+ r_2^{\frac 13} \Big (\frac {r_0}{T+1} \Big)^{\frac 23}.
$$
\end{itemize}	

In summary, 
$$
\frac{1}{T+1}\sum_{t=0}^T \E\Big[\norm{\nabla f(\bar \x^{(t)})}^2 \Big] = \Om \Big(
\frac{\sigma}{\sqrt{nT}} + \frac {\beta^{\frac 23}\sigma^{\frac 23}}{(1-\beta)^{\frac 13}T^{\frac 23}}
+\frac {\beta^{\frac 23}b^{\frac 23}}{(1-\beta)^{\frac 13} T^{\frac 23}}
+\frac {\beta}{T(1-\beta)}
\Big).$$

~

~

~


\textbf{Strongly convex case.}

We assume that $f_i(\x)$ is strongly convex for any $i$, i.e., there exists a constant $\mu$ such that
$$
f_i(\y) \ge f_i(\x) + \langle \nabla f_i(\x), \y - \x \rangle +\frac {\mu}{2} \norm{\y-\x}^2, ~~\forall x, y \in \R^d.
$$

Following a similar analysis as \cite{Koloskova2020AUT}, we have the following descent lemma.
\begin{lemma}
\label{lem:strdescent}
(DESCENT LEMMA)
Let Assumptions A.1-A.3 hold, and $f_i(\x)$  be  $\mu$-strongly convex for all $i$. 
Suppose that $\W^{(t)}$ is doubly stochastic for any $t$.
If $\gamma < 1/(4L)$, then
\begin{equation*}
\begin{aligned}
\E \Big[ \norm{\bar \x^{(t)} - \x^*}^2 \Big] \le &
\big(1- \frac {\gamma \mu}{2} \big)\E \Big[ \norm{\bar \x^{(t-1)} - \x^*}^2 \Big]
-\gamma \E \big( f(\bar \x^{(t-1)}) - f(\x^*)\big)  \\
&+ \frac{5\gamma L}{2n}\E \Big[ \norm{ \X^{(t-1)} - \bX^{(t-1)} }_F^2 \Big] 
+ \frac {\gamma^2 \sigma^2}{n}.
\end{aligned}		
\end{equation*}	
\end{lemma}	

Moreover, we have the following consensus lemma.
\begin{lemma}
\label{lem:strcons}
(EGODIC CONSENSUS LEMMA)
Let Assumptions A.1- A.3 hold, and $f_i(\x)$  be  $\mu$-strongly convex for all $i$. 
Suppose that $\W^{(t)}$ is doubly stochastic for any $t$.
If $\gamma < 1/(4L)$, then
\begin{equation*}
\begin{aligned}
\frac {1}{H_T} \sum_{t=0}^T h^{(t)} \norm{\X^{(t)} - \bX^{(t)}}_F^2 \le 
\frac {48 n \beta^2 \gamma^2 L}{(1-\beta)^2 H_T} \sum_{t=0}^T h^{(t)} \E\big( f(\bar \x^{(t)})  -f(\x^*) \big)
+\frac{2n \beta^2\gamma^2}{1-\beta}\Big(\frac {3b^2}{1-\beta}+\sigma^2 \Big)
\end{aligned}		
\end{equation*}	
where the positive weights satisfy 
$$
h^{(t)} \le h^{(s)} \Big(1+ \frac {1-\beta}{2} \Big)^{t-s},~~ \forall t \ge 0, ~\forall 0\le s \le t,
$$
and $H_T = \sum_{t=0}^T h^{(t)}$.
\end{lemma}	

\emph{Proof.}
By a similar analysis of  (\ref{onestepdes:inenonconv}), it holds for convex $f_i$ that
\begin{equation}
\begin{aligned}
\label{onestepdes:ineconv}
\E \Big[ \norm{ \X^{(t+1)} - \bX^{(t+1)}}_F^2 \Big] \le 
\frac {3\gamma^2 \beta^2 L^2}{1-\beta}\sum_{s=0}^t \beta^{t-s} \E \Big[\norm{\X^{(s)} - \bX^{(s)}}_F^2\Big]& \\
+\frac {6 n\gamma^2 \beta^2}{1-\beta}  \sum_{s=0}^t  \beta^{t-s} \E\big[f(\bar \x^{(s)}) - f(\x^*) \big]
+\frac{2 n \gamma^2 \beta^2}{1-\beta}  \Big(\sigma^2 + \frac {3 b^2}{1-\beta} \Big)&.
\end{aligned}		
\end{equation}	
For simplification, we define 
$$
D_1^{(t)}=\E \Big[\norm{ \X^{(t)} - \bX^{(t)}}_F^2 \Big],~~
D_3^{(t)}=\E \big[f(\bar \x^{(s)}) - f(\x^*) \big],
$$
and moreover,
$$
c_1=\frac {3\gamma^2 \beta^2 L^2}{1-\beta},~~
c_3=\frac{2 n \gamma^2 \beta^2}{1-\beta}  \Big(\sigma^2 + \frac {3 b^2}{1-\beta} \Big),~~
c_4=\frac {6 n\gamma^2 \beta^2}{1-\beta} ,~~
$$
By taking the weighted summation over $t$ for (\ref{onestepdes:ineconv}), we derive
$$
\sum_{t=1}^T h^{(t)} D_1^{(t)} \le c_1 \sum_{t=1}^T h^{(t)}\Big(\sum_{s=0}^{t-1} \beta^{t-1-s} D_1^{(s)} \Big)
+c_4 \sum_{t=1}^T h^{(t)} \Big(\sum_{s=0}^{t-1} \beta^{t-1-s} D_3^{(s)} \Big)
+c_3 \Big(\sum_{t=1}^T h^{(t)}  \Big).
$$

Note that $h^{(t)}\le h^{(s)} \big(1+ \frac {1-\beta}{2} \big)^{t-s}$. Then
\begin{equation*}
\begin{aligned}
\sum_{t=1}^T h^{(t)} \Big(\sum_{s=0}^{t-1} \beta^{t-1-s} D_1^{(s)} \Big) \le 
\Big(1+ \frac {1-\beta}{2} \Big)\sum_{t=1}^T \sum_{s=0}^{t-1} \Big[\Big(1+ \frac {1-\beta}{2} \Big)\beta\Big]^{t-1-s} h^{(s)} D_1^{(s)}
\end{aligned}		
\end{equation*}	

Clearly, $\big(\frac {1-\beta}{2} \big)\beta \le \frac {1+\beta}{2}$, and as a result,
\begin{equation*}
\begin{aligned}
\sum_{t=1}^T h^{(t)}& \Big(\sum_{s=0}^{t-1} \beta^{t-1-s} D_1^{(s)} \Big) \le 
\Big(1+ \frac {1-\beta}{2} \Big)\sum_{t=1}^T \sum_{s=0}^{t-1} \Big(\frac {1+\beta}{2} \Big)^{t-1-s} h^{(s)} D_1^{(s)} \\
&\le \Big(1+ \frac {1-\beta}{2} \Big)\sum_{s=0}^{T-1}  h^{(s)} D_1^{(s)} \sum_{t=s+1}^{T} \Big(\frac {1+\beta}{2} \Big)^{t-1-s}
\le \frac {4}{1-\beta} \sum_{t=0}^{T}  h^{(t)} D_1^{(t)}.
\end{aligned}		
\end{equation*}	


Similarly, we have
\begin{equation*}
\begin{aligned}
\sum_{t=1}^T h^{(t)} \Big(\sum_{s=0}^{t-1} \beta^{t-1-s} D_3^{(s)} \Big) 
\le \frac {4}{1-\beta} \sum_{t=0}^{T}  h^{(t)} D_3^{(t)}.
\end{aligned}		
\end{equation*}	

Therefore,
$$
\sum_{t=0}^T h^{(t)} D_1^{(t)} \le 
\frac {4c_1}{1-\beta} \sum_{t=0}^{T}  h^{(t)} D_1^{(t)}
+\frac {4c_4}{1-\beta} \sum_{t=0}^{T}  h^{(t)} D_3^{(t)}
+c_3 \Big(\sum_{t=1}^T h^{(t)}  \Big).
$$
If $\gamma \le \frac {1-\beta}{5\beta L}$, then $1-\frac{4c_1}{1-\beta} \ge \frac 12$. Consequently,
$$
\frac{1}{H_T} \sum_{t=0}^T h^{(t)} D_1^{(t)} \le 
+\frac {8c_2}{(1-\beta)H_T} \sum_{t=0}^{T}  h^{(t)} D_3^{(t)}
+2c_3,
$$
where $H_T = \sum_{t=0}^T h^{(t)}$. The proof is completed.

~

\textbf{Convergence Theorem}
\begin{theorem}
Let Assumptions A.1- A.3 hold, and $f_i(\x)$  be  $\mu$-strongly convex for all $i$. 
Suppose that $\W^{(t)}$ is doubly stochastic for any $t$.
If $\gamma=\Om\big(\ln(nT)/T\big)$, 
then
$$
\frac {1}{H_T} \sum_{t=0}^T h^{(t)}\Big(\E \big(f(\bar \x^{(t)})  \big) - f(\x^*) \Big) =
\tilde{\Om}\Big( \frac{\sigma^2}{nT} + \frac{\beta^2 \sigma^2}{(1-\beta)T^2} + \frac{\beta^2 b^2}{(1-\beta)^2 T^2}
+\exp\big(-(1-\beta)T\big) \Big)
$$	
where $\tilde{\Om}$ hides logarithm.
\end{theorem}

\emph{Proof.}
It follows from Lemma \ref{lem:strdescent} that
\begin{equation*}
\begin{aligned}
\E \Big[ \norm{\bar \x^{(t)} - \x^*}^2 \Big] \le &
\big(1- \frac {\gamma \mu}{2} \big)\E \Big[ \norm{\bar \x^{(t-1)} - \x^*}^2 \Big]
-\gamma \E \big( f(\bar \x^{(t-1)}) - f(\x^*)\big)  \\
&+ \frac{5\gamma L}{2n}\E \Big[ \norm{ \X^{(t-1)} - \bX^{(t-1)} }_F^2 \Big] 
+ \frac {\gamma^2 \sigma^2}{n}.
\end{aligned}		
\end{equation*}	

Taking weighted over $t$, it holds that
\begin{equation*}
\begin{aligned}
\frac {1}{H_T}\sum_{t=0}^T h^{(t)} \E \big( f(\bar \x^{(t-1)}) - f(\x^*)\big) \le 
\frac {1}{\gamma H_T}\sum_{t=0}^T h^{(t)} \Big(\big(1- \frac {\gamma \mu}{2} \big)\E \Big[ \norm{\bar \x^{(t-1)} - \x^*}^2 \Big]& \\
-\E \Big[ \norm{\bar \x^{(t)} - \x^*}^2 \Big] \Big) 
+ \frac {5L}{2nH_T}\sum_{t=0}^T h^{(t)} E \Big[ \norm{\bar \x^{(t)} - \x^{(t)}}^2 \Big]
+ \frac {\gamma \sigma^2}{n}&.
\end{aligned}		
\end{equation*}	

We define $h^{(t)}=\big(1- \frac {\gamma \mu}{2} \big)h^{(t+1)}$, and then  
\begin{equation*}
\begin{aligned}
\frac {1}{H_T}\sum_{t=0}^T h^{(t)} \E \big( f(\bar \x^{(t-1)}) &- f(\x^*)\big) \le 
\frac {h^{(0)}}{\gamma H_T}\E \Big[ \norm{\bar \x^{(0)} - \x^*}^2 \Big] \\
&+ \frac {5L}{2nH_T}\sum_{t=0}^T h^{(t)} E \Big[ \norm{ \X^{(t-1)} - \bX^{(t-1)} }_F^2 \Big] 
+ \frac {\gamma \sigma^2}{n}.
\end{aligned}		
\end{equation*}	

If $\gamma \le \frac{1-\beta}{3\mu}$, then $\frac {1}{1- \frac {\gamma \mu}{2}} \le 1 + \frac {1-\beta}{2}$.
Recalling Lemma \ref{lem:strcons} gives
\begin{equation*}
\begin{aligned}
\frac {1}{H_T}\sum_{t=0}^T h^{(t)} &\E \big( f(\bar \x^{(t-1)}) - f(\x^*)\big) \le
\frac {h^{(0)}}{\gamma H_T}\E \Big[ \norm{\bar \x^{(0)} - \x^*}^2 \Big]
+ \frac {\gamma \sigma^2}{n} \\
&+ \frac {120 n \beta^2 \gamma^2 L}{(1-\beta)^2 H_T} \sum_{t=0}^T h^{(t)} \E \big[f(\bar \x^{(t-1)}) - f(\x^*)\big]
+ \frac{5 \beta^2\gamma^2L}{1-\beta}\Big(\frac {3b^2}{1-\beta}+\sigma^2 \Big).
\end{aligned}		
\end{equation*}	

If $\gamma \le \frac {1-\beta}{16\beta L}$, then  $\frac {120 n \beta^2 \gamma^2 L}{(1-\beta)^2} \le \frac 12$. It holds that
\begin{equation*}
\begin{aligned}
\frac {1}{H_T}\sum_{t=0}^T h^{(t)} &\E \big( f(\bar \x^{(t-1)}) - f(\x^*)\big) \le
\frac {2h^{(0)}}{\gamma H_T}\E \Big[ \norm{\bar \x^{(0)} - \x^*}^2 \Big]  \\
&+ \frac {2\gamma \sigma^2}{n}
+ \frac{10 \beta^2\gamma^2L}{1-\beta}\Big(\frac {3b^2}{1-\beta}+\sigma^2 \Big).
\end{aligned}		
\end{equation*}		

Since $H_T \ge h_T = h_0(1- \frac{\gamma \mu}{2})$, we have
\begin{equation*}
\begin{aligned}
\frac {1}{H_T}\sum_{t=0}^T h^{(t)} &\E \big( f(\bar \x^{(t-1)}) - f(\x^*)\big) \le
\frac {2h^{(0)}}{\gamma}\E \Big[ \norm{\bar \x^{(0)} - \x^*}^2 \Big] \exp{\big(- \frac {\gamma \mu T}{2}\big)}  \\
&+ \frac {2\gamma^2 \sigma^2}{n}
+ \frac{10 \beta^2\gamma^2L}{1-\beta}\Big(\frac {3b^2}{1-\beta}+\sigma^2 \Big).
\end{aligned}		
\end{equation*}		

Take 
$$
\gamma = \min  \Big\{ \frac{1}{4L}, \frac{1-\beta}{3\mu}, \frac{1-\beta}{16\beta L}, 
\frac{2}{\mu T}\ln{\Big(\frac{n\mu T^2}{\sigma^2}  \E \Big[ \norm{\bar \x^{(0)} - \x^*}^2 \Big] \Big)}   \Big\}.
$$
By a similar procedure for non-convex case, it can be show that
$$
\frac {1}{H_T} \sum_{t=0}^T h^{(t)}\Big(\E \big(f(\bar \x^{(t)})  \big) - f(\x^*) \Big) =
\tilde{\Om}\Big( \frac{\sigma^2}{nT} + \frac{\beta^2 \sigma^2}{(1-\beta)T^2} + \frac{\beta^2 b^2}{(1-\beta)^2 T^2}
+\exp\big(-(1-\beta)T\big) \Big).
$$	
